Specification Construction Using Behaviours, Equivalences, and SMT Solvers

We propose a method to write and check a specification including quantifiers using behaviors, i.e., input-output pairs. Our method requires the following input from the user: (1) answers to a finite number of queries, each of which presents some behavior to the user, who responds informing whether the behavior is "correct" or not; and (2) an "equivalence" theory (set of formulae), which represents the users opinion about which pairs of behaviors are equivalent with respect to the specification; and (3) a "vocabulary", i.e., a set of formulae which provide the basic building blocks for the specification to be written. Alternatively, the user can specify a type theory and a simple relational grammar, and our method can generate the vocabulary and equivalence theories. Our method automatically generates behaviors using a satisfiability modulo theory solver. Since writing a specification consists of formalizing ideas that are initially informal, there must, by definition, be at least one "initial" step where an informal notion is formalized by the user in an ad hoc manner. This step is the provision of the equivalence theory and vocabulary; we call it the primitive formalization step. We contend that it is considerably easier to write an equivalence theory and vocabulary than to write a full-blown formal specification from scratch, and we provide experimental evidence for this claim. We also show how vocabularies can be constructed hierarchically, with a specification at one level providing vocabulary material for the next level.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%\RequirePackage{mathabx}

\RequirePackage{relsize}
\RequirePackage{fancyvrb}
\RequirePackage{ifthen}
\RequirePackage{multirow}

\RequirePackage{amsmath}
%\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{latexsym}

\RequirePackage{xspace}
\RequirePackage{url}

\usepackage[pdftex]{graphicx}
\RequirePackage{color}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPECCHECK SPECIFIC SYMBOLS
\newcommand{\MATH}[1]{\ensuremath{#1}\xspace}

\newcommand{\aff}{[\ff,\ldots,\ff]} 
\newcommand{\att}{[\tt,\ldots,\tt]}  
\newcommand{\arr}[1]{[#1]}  


%% Algorithm names
\newcommand{\mkAdeq}{\textsf{MakeAdequate}}
\newcommand{\constFor}{\textsf{ConstructFormula}}

\newcommand{\checkAd}{\textsf{CheckAdequacy}}
\newcommand{\checkAdA}[1]{\textsf{CheckAdequacy}$(#1)$}

%% theories
\newcommand{\gth}{\MATH{\gamma}}                              % generic theory
\newcommand{\tth}{\MATH{\tau}}                                     % type theory
\renewcommand{\eth}{\MATH{\varepsilon}}                       % equivalence theory
\newcommand{\eps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\voc}{\MATH{\mathit{\nu}}}                        % vocabulary

\newcommand{\Vt}{\MATH{V_\tau}}                                   % assignment to type theory                            
\newcommand{\Ve}{\MATH{V_\varepsilon}}                        % assignment to equivalence theory                            
\newcommand{\Vv}{\MATH{V_\voc}}                                  % assignment to vocabulary

%% bounded theories
\newcommand{\ethb}[1]{\MATH{\varepsilon_{#1}}}             % bounded equivalence theory
\newcommand{\vocb}[1]{\MATH{\mathit{\nu}_{#1}}}           % bounded vocabulary

\newcommand{\Veb}[1]{\MATH{V_{\varepsilon_{#1}}}}         % assignment to bounded equivalence theory 
%\newcommand{\Veb}[1]{\MATH{V_{\varepsilon}^{#1}}}                   % assignment to bounded equivalence theory 

             
\newcommand{\Vvb}[1]{\MATH{V_{\voc}^{#1}}}                         % assignment to bounded vocabulary

%% metasyntax
\newcommand{\ethm}{\MATH{\hat{\varepsilon}}}
\newcommand{\ethmb}[1]{\MATH{\hat{\varepsilon}_{#1}}}



%% formulae
\newcommand{\Sp}{\ensuremath{\mathcal{S}}\xspace}         % specification
\newcommand{\cfor}[1]{\MATH{\mathit{cfor}[#1]}}               % correction formula for inadequate vocabulary
\newcommand{\for}[1]{\MATH{\mathit{fm}(#1)}}                     % formula corresponding to an assignment
\newcommand{\Fo}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Pre}{\ensuremath{P}}                                % precondition
\newcommand{\Post}{\ensuremath{Q}}                              % postcondition

\newcommand{\lft}{\ensuremath{\mathcal{left}}\xspace}
\newcommand{\rgt}{\ensuremath{\mathcal{right}}\xspace}
\newcommand{\eina}{\ensuremath{\mathcal{eina}}\xspace}

%% model theory
\renewcommand{\th}{\MATH{\beta}}                                 % threshold for satisfiability checking
\newcommand{\md}[1]{\MATH{[ #1 ]}}                               % set of points satisfying a formula ``model''
%\newcommand{\md}[1]{\ensuremath{[ #1 ]}\xspace}
\newcommand{\Bool}{\set{\tt,\ff}}                                % the Boolean type
\newcommand{\Part}{\ensuremath{\set{\vtt,\vff}}\xspace}          % the partition of D
\newcommand{\asg}{\ensuremath{\sigma}}                         % assignment, ie state
\newcommand{\beh}{\ensuremath{\sigma}}                         % behavior
\newcommand{\behi}{\ensuremath{\beh_i}}                      % input behavior
\newcommand{\beho}{\ensuremath{\beh_o}}                    % output behavior
\newcommand{\Beh}{\ensuremath{\Sigma}\xspace}             % the set of behaviors
\newcommand{\D}{\ensuremath{\MATH{D}}}
\newcommand{\U}{\ensuremath{\MATH{U}}}



%% logic
\newcommand{\IL}{\ensuremath{L_{\omega_{1},\omega}}\xspace}

%% variables
\newcommand{\sv}{x}   % vars used in specification

%% ranges




%% old?
\newcommand{\E}{\mathcal{E}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\redTo}{\ensuremath{\rhd}}
\newcommand{\FS}{\mathcal{F}}
\newcommand{\PS}{\mathcal{P}}
\newcommand{\M}{\mathcal{M}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END SPECCHECK SPECIFIC SYMBOLS





%%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations
\newcommand{\assig}{\ensuremath{\sigma}}
\newcommand{\sg}{\ensuremath{\sigma}}
\newcommand{\tf}{\ensuremath{\{\tt, \ff\}}}
\newcommand{\form}{\ensuremath{\mathit{form}}}
\newcommand{\vphi}{\ensuremath{\varphi}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%% Lists
\newcommand{\be}{\begin{itemize}}
\newcommand{\ee}{\end{itemize}}
\newcommand{\bdn}{\begin{description}}
\newcommand{\edn}{\end{description}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\renewcommand{\i}{\item}

\newenvironment{closeitemize}{\begin{list}%
{$\bullet$}%
{\setlength{\itemsep}{-0.2\baselineskip}%
\setlength{\topsep}{0.2\baselineskip}}}%
{\end{list}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISC

\newcommand{\remove}[1]{}

%\newcommand{\case}[2]{\vspace{1.5ex} \noindent \textit{Case} #1: \emph{#2}.}
\newcommand{\scase}[2]{\vspace{1.5ex} \noindent \textit{Subcase} #1: #2.}
\newcommand{\sscase}[2]{\vspace{1.0ex} \noindent \textit{Subsubcase} #1: #2.}

%\newcommand{\defn}[1]{\textit{#1}}
\newcommand{\defi}[1]{\textit{#1}:}

\newcommand{\lb}{\linebreak}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES AND THEOREMS


\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\renewcommand{\thefootnote}{\arabic{footnote}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text
\newcommand{\smpage}{\noindent \parbox{\textwidth}}
\newcommand{\samep}{\parbox{\textwidth}}   % put onto the same page


\newcommand{\mathid}[1]{\ensuremath{\mathit{#1}}\xspace}

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\ul}{\underline}
\newcommand{\bs}{\bigskip}
%\newcommand{\ms}{\medskip}
%\renewcommand{\ss}{\smallskip}

\newcommand{\bfg}{\begin{figure}}
\newcommand{\efg}{\end{figure}}

\renewcommand{\ss}{\smallskip}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}


\newcommand{\intr}{\empi}
\newcommand{\intrdef}{\emph}

\newcommand{\emp}[1]{\textbf{#1}}
\newcommand{\empp}[1]{\emph{#1}}
\newcommand{\empb}[1]{\textbf{#1}}
\newcommand{\empi}[1]{\textit{#1}}
\newcommand{\empbi}[1]{\textbf{\textit{#1}}}

\newcommand{\ind}{\hspace*{3.0em}}

%%%%%From Nancy's book directory:  This spaces the symbols within a
%%%%%word nicely, in math mode.
\newcommand{\ms}[1]{%
        \relax\ifmmode
                \mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}%
        \else
                $\mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}$%
        \fi
}


\newcommand{\cmnt}{\`//}


%%%%%%%%%%%%%%%%%%%%%%% GENERAL MATH SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Adj}{\mathop{\rm Adj}\nolimits}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\card}[1]{\left| #1\right|}
\newcommand{\ar}{\rightarrow}
%\newcommand{\ar}{\longrightarrow}
\newcommand{\al}{\alpha}
\renewcommand{\b}[1]{\overline{#1}}
\newcommand{\cat}{\mathbin{\frown}}
\newcommand{\choice}{\mbox{$[\hspace*{-1.0pt}]$}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\renewcommand{\d}{\, . \,}      % separator in quantified formulae
\newcommand{\df}{\triangleq}
%\newcommand{\df}{\mbox{$\:\stackrel{\rm df}{=\!\!=}\:$}}
\newcommand{\dn}{\mbox{$\hspace{-0.1em}\downarrow\hspace{-0.1em}$}}
\newcommand{\Ex}{\mathop{\rm Ex}}
\newcommand{\es}{``"}   %empty string
\newcommand{\expect}[1]{{\rm E}\left[ #1 \right]}
\newcommand{\expectsq}[1]{{\rm E}^2\left[ #1 \right]}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\renewcommand{\ge}{\geqslant}
\newcommand{\given}{\mid}
\newcommand{\halfind}{\hspace*{1.5em}}
\newcommand{\ifof}{\Longleftrightarrow} % logical equivalence
\newcommand{\img}{\mathrm{Image}}
\newcommand{\ints}{\cap}
\renewcommand{\l}{\ell}
\newcommand{\la}[1]{\mbox{$\, \stackrel{#1}{\rightarrow} \,$}}
\renewcommand{\le}{\leqslant}
\newcommand{\lra}{\mbox{$\longrightarrow$}}
%\newcommand{\mod}{\ \mathrm{mod}\ }
\newcommand{\oneton}{\{1,\,\ldots, n\}}
\newcommand{\n}{\ensuremath{[1:n]}} 
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\pair}[2]{\ensuremath{(#1, #2)}}
\newcommand{\pind}{\hspace*{3.0em}}
\newcommand{\pj}{\!\upharpoonright\!}
\newcommand{\proj}{\pj}
\newcommand{\preimg}{\mathrm{PreImage}}
\newcommand{\pl}{\!\parallel\!}
\newcommand{\s}{\mbox{$\hspace{-1pt}-\hspace{-2pt}$}}
\newcommand{\set}[1]{\ensuremath{\{ #1 \}}\xspace}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\seq}{\approx}
\newcommand{\spc}{\mbox{\vspace{-0.25in}}}
\newcommand{\stt}{\ | \ }
\newcommand{\st}[1]{\ensuremath{[ #1 ]}\xspace}
\newcommand{\sub}{\subseteq}
\newcommand{\twodots}{\mathinner{\ldotp\ldotp}}
\newcommand{\tiff}{\textup{\ iff\ }}
\newcommand{\tl}[1]{\mbox{$\tilde{#1}$}}% abbreviated tilde
\newcommand{\tpl}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\un}{\cup}
\newcommand{\union}{\bigcup}
\newcommand{\up}{\mbox{$\hspace{-0.1em}\uparrow\hspace{-0.1em}$}}
\newcommand{\Var}{\mathop{\rm Var}\nolimits}
\newcommand{\variance}[1]{{\rm Var}\left[ #1 \right]}
\newcommand{\w}{\omega}


%%%%%%%%%%%%%%%%%%% Ints, Reals, etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\reals}{{\mathbb R}}
\newcommand{\integers}{{\mathbb Z}}
\newcommand{\naturals}{{\mathbb N}}
\newcommand{\nat}{\naturals}
\newcommand{\nats}{\naturals}
\newcommand{\rationals}{{\mathbb Q}}
\newcommand{\complex}{{\mathbb C}}
\newcommand{\complexes}{{\mathbb C}}



%%%%%%%%%%%%%%%%%%%%%%%%% MATH MACROS AND ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\se}[3]{\ensuremath{#1[#2 .. #3]}}
\newcommand{\se}[3]{\ensuremath{#1[#2 \! : \! #3]}}
%\newcommand{\se}[3]{\ensuremath{#1[#2,\ldots,#3]}}


\newcommand{\ang}[1]{\ifmmode{\left\langle #1 \right\rangle}
   \else{$\left\langle${#1}$\right\rangle$}\fi}
        % the \if allows use outside mathmode,
        % but will swallow following space there!

\newcommand{\struct}[2]{\raisebox{-0.1in}{$\stackrel { \displaystyle
#1} {\scriptstyle #2}\,$}}

\newcommand{\pbx}[2]{\stackrel{\fbox{\begin{Beqnarray*} #1\\.\\.\\.\\#2 \end{Beqnarray*}}}{}}      % proof box

\newcommand{\asrt}[1]{\ensuremath{\{ #1 \}}}

%%%%%%%%%%%%%%%%%%%%%%% Hoare Logic Symbols
\newcommand{\lng}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\htp}[3]{\ensuremath{\{#1\}\,#2\,\{#3\}}}
\newcommand{\htptc}[3]{\ensuremath{\langle#1\rangle\,#2\,\langle#3\rangle}}
\newcommand{\var}{\ensuremath{\varphi}}

\newcommand{\as}[1]{\ensuremath{\{#1\}}}               % partial correctness asserion
%\newcommand{\ts}[1]{\ensuremath{\langle #1 \rangle}}   % termination correctness asserion

\newcommand{\ch}{\mbox{[\hspace{-0.15ex}]}}

\newcommand{\pa}[1]{\{\ensuremath{#1}\}}
%\newcommand{\ta}[1]{$<$#1$>$}
\newcommand{\ta}[1]{$\langle$\ensuremath{#1}$\rangle$}

\newcommand{\pre}[1]{\textsf{Precondition: #1}}
\newcommand{\post}[1]{\textsf{Postcondition: #1}}

\newcommand{\satt}{\equiv}
\newcommand{\sat}{\models}
\newcommand{\satf}{\mbox{\ensuremath{=\hspace*{-5pt}|}}}   % satisfiable - backward turnstile
%\newcommand{\satf}{\mbox{\ensuremath{=\!\!\!\!|}}}   % satisfiable - backward turnstile


\newcommand{\yld}{\vdash}
\newcommand{\yldd}{\equiv}
%\newcommand{\yldd}{\dashv \vdash}






\newcommand{\pc}[1]{{#1}}    %% font for pseudocode
%\newcommand{\pc}[1]{\codetext{#1}}    %% font for pseudocode



%%%%%%%%%%%%%%%%%%%%%%%% JUSTIFY EXAMPLE MACROS
\newcommand{\valpha}{\ensuremath{\mathit{alpha}}}
\newcommand{\numeric}{\ensuremath{\mathit{numeric}}}
\newcommand{\wspace}{\ensuremath{\mathit{wspace}}}
\newcommand{\vnewline}{\ensuremath{\mathit{newline}}}
\newcommand{\blank}{\ensuremath{\mathit{blank}}}
\newcommand{\word}{\ensuremath{\mathit{word}}}
\newcommand{\lline}{\ensuremath{\mathit{line}}}
\newcommand{\para}{\ensuremath{\mathit{para}}}
\newcommand{\numWords}{\ensuremath{\mathit{numWords}}}
\newcommand{\selectWord}{\ensuremath{\mathit{selectWord}}}
\newcommand{\numLines}{\ensuremath{\mathit{numLines}}}


%\RequirePackage{metre}

\newcommand{\nl}{\ensuremath{\backslash n}}
\newcommand{\bl}{\textvisiblespace}
\newcommand{\tx}{tx}



%%%%%%%%%%%%%% MACROS FOR NUMBERED LINES IN CODE TABBING ENVIRONMENT %%%%%%%%%%%%%%%%

\newcounter{lctr}

\newcommand{\li}{\addtocounter{lctr}{1}\arabic{lctr}.}
\newcommand{\lio}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\ensuremath{#1}\\}
\newcommand{\lit}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\ensuremath{#1}\\}
\newcommand{\lih}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\>\ensuremath{#1}\\}

%%%% 2'nd argument is for a commment
\newcommand{\lioc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\ensuremath{#1}\`{#2}\\}
\newcommand{\litc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\ensuremath{#1}\`{#2}\\}
\newcommand{\lihc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\>\ensuremath{#1}\`{#2}\\}




%%%%%%%%%%%%%%%%%%%%%%%%%%% PSEUDOCODE SECTION

\newcommand{\gt}{\ensuremath{:=}}   % assignment
%\newcommand{\gt}{\ensuremath{\leftarrow}}   % assignment
\newcommand{\swap}{\ensuremath{\leftrightarrow}}   % swap two vars

\newcommand{\pseudocode}[1]{\ensuremath{\mathbf{#1}}\xspace}
%\newcommand{\pseudocode}[1]{\ensuremath{\mathbf{#1}\ }}
\newcommand{\pseudocodensp}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\pseudocode}[1]{\mbox{${\bf #1}$}\xspace}

\newcommand{\IFC}[1]{\pseudocode{if}\ (\ensuremath{#1})}
\newcommand{\WHILEC}[1]{\pseudocode{while}\ (\ensuremath{#1})}
\newcommand{\RETURNE}[1]{\pseudocodensp{return}(\ensuremath{#1})}

\newcommand{\IF}{\pseudocode{if}}
\newcommand{\FI}{\pseudocode{fi}}
\newcommand{\THEN}{\pseudocode{then}}
\newcommand{\ELSE}{\pseudocode{else}}
\newcommand{\ELSF}{\pseudocode{else\ if}}
\newcommand{\ENDIF}{\pseudocodensp{endif}}

\newcommand{\WHILE}{\pseudocode{while}}
\newcommand{\ENDWHILE}{\pseudocode{endwhile}}
\newcommand{\FOR}{\pseudocode{for}}
\newcommand{\FORALL}{\pseudocode{forall}}
\newcommand{\FOREACH}{\pseudocode{foreach}}
\newcommand{\CONTINUE}{\pseudocode{continue}}
\newcommand{\ENDFOR}{\pseudocodensp{endfor}}
\newcommand{\DO}{\pseudocode{do}}
\newcommand{\OD}{\pseudocode{od}}

\newcommand{\BEGIN}{\pseudocode{begin}}
\newcommand{\END}{\pseudocode{end}}
\newcommand{\PROC}{\pseudocode{procedure}}
\newcommand{\CALL}{\pseudocode{call}}
\newcommand{\VAL}{\pseudocode{value}}
\newcommand{\VALRES}{\pseudocode{value\!-\!result}}
\newcommand{\RES}{\pseudocode{result}}
\newcommand{\RETURN}{\pseudocodensp{return}}
\newcommand{\DOWNTO}{\pseudocode{downto}}
\newcommand{\TO}{\pseudocode{to}}

\newcommand{\function}{\pseudocode{function}}
\newcommand{\operation}{\pseudocode{operation}}

\newcommand{\newo}{\pseudocode{new}}
\renewcommand{\int}{\pseudocode{int}}

\newcommand{\skipp}{\pseudocode{skip}}







%%%%%%%%%%%%%%%%%%%%%%%%%%%% Boolean Constants




\newcommand{\T}{\mbox{\rm T}}
\newcommand{\F}{\mbox{\rm F}}
\newcommand{\Fa}{\mbox{\rm F}}

\newcommand{\true}{\ensuremath{\mathit{true}}}
\renewcommand{\tt}{\ensuremath{\mathit{tt}}}
\newcommand{\vtt}{\ensuremath{\mathit{vtt}}\xspace}
%\newcommand{\true}{\mbox{\textsc{true}}\xspace}

\newcommand{\false}{\ensuremath{\mathit{false}}}
\newcommand{\ff}{\ensuremath{\mathit{ff}}}
\newcommand{\vff}{\ensuremath{\mathit{vff}}\xspace}
%\newcommand{\false}{\mbox{\textsc{false}}\xspace}

%\newcommand{\TT}{\top}
%\newcommand{\FF}{\bot}

\newcommand{\TT}{\mathit{true}}
\newcommand{\FF}{\mathit{false}}

\newcommand{\andw}{\mbox{ and }}

%\newcommand{\ANDW}{\mbox{\bf and \xspace}}
%\newcommand{\OR}{{\bf or} }
%\newcommand{\NOT}{{\bf not} }




%%%%%%%%%%%%%%%%%%%%%%%%% Boolean Connectives

\renewcommand{\iff}{\equiv}
%\renewcommand{\iff}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\ev}{\equiv}
%\newcommand{\implies}{\Rightarrow}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QUANTIFIERS

\newcommand{\qt}[3]{#1\,#2\,#3}
\newcommand{\qtr}[4]{(#1\,#2 : #3 : #4)}

\newcommand{\Q}{\mbox{${\bf Q}$}\xspace}
\newcommand{\q}{\mbox{${\bf q}$}\xspace}

%% quantifiers
\newcommand{\AND}{\bigwedge}
\newcommand{\INTER}{\bigcap}
\newcommand{\OR}{\bigvee}
\newcommand{\UN}{\bigcup}
\newcommand{\SUM}{\Sigma}
%\newcommand{\INT}{\bigcap}

%% Logical Quantifiers
\newcommand{\fa}{\ensuremath{\forall\,}}
%\newcommand{\fa}{\mbox{${\mathbf{\forall}}$}\xspace}
\newcommand{\ex}{\ensuremath{\exists\,}}
%\newcommand{\ex}{\mbox{${\mathbf{\exists}}$}\xspace}

\newcommand{\LQ}{\mbox{${\bf LQ}$}\xspace}


%% Arithmetic Quantifiers
%\renewcommand{\S}{\Sigma\,}
%\renewcommand{\S}{\mbox{${\mathbf{\Sigma}}$}\xspace}
\renewcommand{\P}{\Pi\,}
\newcommand{\N}{\ensuremath{\mathrm{N}\,}}
\newcommand{\AQ}{\ensuremath{\mathrm{AQ}\,}}
\newcommand{\MAX}{\ensuremath{\mathrm{MAX}\,}}
\newcommand{\MIN}{\ensuremath{\mathrm{MIN}\,}}


%%%%%%%%%%%%%%%%% ENVIRONMENTS
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}

%%%%%%%%%%%%%%%%% EQUATION ENVIRONMENTS
\newcommand{\beqn}{\begin{centeqn}}
\newcommand{\eeqn}{\end{centeqn}}
\newcommand{\beqnnbsp}{\begin{centeqn-nbsp}}
\newcommand{\eeqnnbsp}{\end{centeqn-nbsp}}
\newcommand{\bleqn}[1]{\begin{centlabeqn}{#1}}
\newcommand{\eleqn}{\end{centlabeqn}}
\newcommand{\bleqnnbsp}[1]{\begin{centlabeqn-nbsp}{#1}}
\newcommand{\eleqnnbsp}{\end{centlabeqn-nbsp}}

\newenvironment{centeqn}	% centered equation environment
   {{\ss\\ \hspace*{\fill}}}
   {\hspace*{\fill}\ss\\}

\newsavebox{\EqnLabel}
\newenvironment{centlabeqn}[1]	% centered labeled equation environment
   {\sbox{\EqnLabel}{#1}
    {\medskip\\ \hspace*{\fill}}
   }
   {\hfill{\makebox[0in][r]{\usebox{\EqnLabel}}}\medskip\\}

\newenvironment{centeqn-nbsp} % centered equation - no vertical space at the bottom
   {{\medskip\\ \hspace*{\fill}}}
   {\hspace*{\fill}}




%%%%%%%%%%%%%%%% SpecCheck Specific macros

\newcommand{\cd}[1]{{\small\texttt{#1}}}
\newcommand{\cci}[1]{\mbox{\textup{\texttt{#1}}}}
%\newcommand{\cci}[1]{{\small\texttt{#1}}}
%\newcommand{\chci}[1]{`\cci{#1}'}
\newcommand{\chci}[1]{\cci{#1}}

\newcommand{\good}{\cci{good}\xspace}
\newcommand{\bad}{\cci{bad}\xspace}
\newcommand{\dc}{\cci{dontCare}\xspace}
\newcommand{\tgood}{\tiny\texttt{good}\xspace}
\newcommand{\tbad}{\tiny\texttt{bad}\xspace}
\newcommand{\tdc}{\tiny\texttt{dontCare}\xspace}

\newcommand{\ord}{\sqsubseteq}
\newcommand{\ordne}{\sqsubset}

\newcommand{\white}{\ensuremath{\mathit{white}}\xspace}
\newcommand{\black}{\ensuremath{\mathit{black}}\xspace}

\newcommand{\ls}{\cd{ls}}
\newcommand{\af}{f}



\newcommand{\vit}{{\cal T}_I}
\newcommand{\vst}{{\cal T}_S}
\newcommand{\vocrm}{\mathit{voc}_R^M}
\newcommand{\tp}{\mathit{type}}
\newcommand{\tll}{\mathit{tail}}
\newcommand{\hdd}{\mathit{head}}


==> type.tex <==
from the user, we extend
this set with $N$ additional variables to be used 
in index terms.  
%We consider theory ${\cal T}$ to be the set of the smallest expressions in the
%QF-EUF theory derivable from  $\exists\forall_i\tau$. 
%Boolean formulas over the theory ${\cal T}$ can express
%$\exists\forall_i\tau$. 
Consider $\exists\forall_i\tau^K$ where only free variables 
from $X$, and with
at most $N$-depth universal quantifiers. 
Since $\exists\forall_i\tau^K$  is a subset 
of $\exists\forall_i\tau^K$, then   
the satisfiability of $\exists\forall_i\tau^K$ is reducible to the QF-EUF
theory ${\cal T}^K$. 
Consider $\tau$ to be the smallest Boolean formulae in ${\cal T}^K$,
$\tau$ is finite and all its elements are of size $\le K$. 
%
Furthermore $\satf D/\tau$ is decidable since the Boolean formulae over $\tau$
are all in QF-EUF. 

We propose the use of $\tau$ derived from the array property theory along 
with $D/\tau$ to judge the adequacy of the vocab. 
Our method to derive a finite and equisatisfiable theory 
applies to other decidable theories such as the 
decidable fragment of the sequence theory proposed by ~\cite{Furia2010}. 




%In the following we
%propose a quantifier free type theory $\tau^K$ and 
%a quantified extension $\exists\forall_i\tau^K$ that
%is subsumed by the decidable array property theory defined in ~\cite{Brdly06}.
%The thoery $\tau^K$ includes scalars, indices, and arrays where index and
%scalar terms are shorter than $K$ ($K$ is the
%maximum number of arithmetic and indexing operations allowed in one term).
%The intuition behind the proof of decidablity of the quantified formulae is to
%limit universal qantification to index variables and expand universal
%quantifications as conjunctions over the finite set of index terms.
%Existensially quandtified variables are skolemized as usual.
%The resulting formulae are quantifier free, equality, and uninterpreted
%function theory formulae with an NP-complete decision procedure~\cite{Brdly06}.
%
%{\bf Similarly, we can propose a type theory subsumed by the sequence
%property theory based on concatenation theory. by TODO: we can also propose
%a theory that is subsumed by ~\cite{Furia2010}}.
%
%Let $C=\{c_1,c_2,\ldots,c_N\}$ be a set of constants, 
%$X=\{x_1,x_2,\ldots,x_n\}$ be a set of scalar variables, and
%$A=\{a_1,a_2,\ldots,a_m\}$ be a set of array variables. 
%Let $\Sigma=\{<,=,[~],+,-\}$ be the set of operators allowed
%in the clauses of $\tau^K$ that denote less than, equality, array
%indexing (array read), addition, and subtraction, respectively.
%We do not need the array write operator from ~\cite{Brdly06} since our target
%here is to construct a specification.
%
%The relation $R\subset (X\cup C \cup A) \times (X \cup C \cup A) \times \Sigma$ 
%defines the dependency relation and the operators allowed amongst the variables.
%Let $\vit$ and $\vst$ denote index and scalar terms of length
%smaller than $K$, respectively. 
%
%The user must have reasonable knowledge of variable names,
%types, and operations relating the variables.
%The user provides $C$,$X$, and $A$
%explicitly and then provides $R$ via filling a matrix with values
%from $\Sigma$. 
%
%Let 
%$\hdd: \vit \cup \vst \cup \tau \mapsto X\cup A \cup C$ and
%$\tll: \vit \cup \vst \cup \tau \mapsto X\cup A \cup C$,
%be two helper functions that return the first and last variable or constant
%in the text of a term or 
%a clause in $\tau$, respectively.
%\begin{enumerate}
%\item\label{i:vit} Index terms. 
%\begin{enumerate}
%    \item\label{ii:y} $y \in \vit$ and $\hdd(y) = \tll(y) = y$, 
%        given that $y \in X\cup C$ and $\exists a \in A. (y,a,[])\in R$.
%    \item\label{ii:asize} $|a| \in \vit$ and $\hdd(a) = \tll(a) = a$, 
%        given that $a \in A$. 
%    \item\label{ii:aat} $a[t] \in \vit$ and $\hdd(a[t])=\tll(a[t]) = a$, 
%        given that $a\in A, t \in \vit$,
%        $(a,\hdd(t),[]) \in R$.
%        and $\exists a_1 \in A. (a,a_1,[])\in R$.
%    \item\label{ii:circ} $(t_1 \circ t_2) \in \vit$, 
%        $\hdd(t_1 \circ t_2)=\hdd(t_1)$ and $\tll(t_1 \circ t_2)=\tll(t_2)$, 
%        given that $t_1,t_2\in \vit$, $\circ \in \{+,-\}$, 
%        and $(\tll(t_1),\hdd(t_2),\circ) \in R$.
%\end{enumerate}
%
%\item\label{i:vst} Scalar Terms. 
%\begin{enumerate}
%    \item\label{ii:c} $c \in \vst$ and $\hdd(c) = \tll(c) = c$, 
%        given that $c \in C$.
%    \item\label{ii:x} $x \in \vst$ and $\hdd(x) = \tll(x) = x$, 
%        given that $x\in X$.
%    \item\label{ii:a} $a[t] \in \vst$ and $\hdd(a[t])=\tll(a[t]) = a$, 
%        given that $a \in A, t\in \vit$, 
%        and $(a,\hdd(t),[]) \in R$.
%    \item\label{ii:scirc} $(t_1 \circ t_2) \in \vst$, $\hdd(t_1 \circ
%t_2)=\hdd(t_1)$ and $\tll(t_1 \circ t_2)=\tll(t_2)$, 
%        given that $t_1,t_2\in \vst$, $\circ \in \{+,-\}$, 
%        and $(\tll(t_1),\hdd(t_2),\circ) \in R$.
%\end{enumerate}
%
%\item\label{i:idxbound} Index bound terms $\tau^K_b$
%\begin{enumerate}
%    \item\label{ii:ibterm} $(t_1 \circ t_2) \in \tau$, 
%    $\hdd(t_1 \circ t_2)=\hdd(t_1)$ and
%    $\tll(t_1 \circ t_2)=\tll(t_2)$, 
%    given that $t_1,t_2\in \vit$, $\circ \in \{\le,=\}$,  
%        and $(\tll(t_1),\hdd(t_2),\circ) \in R$.
% \end{enumerate}
% \item\label{i:idxbound} Scalar property terms $\tau^K_s$
% \begin{enumerate}
%    \item\label{ii:tsc} $(t_1 \circ t_2) \in \tau^K_s$, 
%        $\hdd(t_1 \circ t_2)=\hdd(t_1)$ and
%        $\tll(t_1 \circ t_2)=\tll(t_2)$, 
%        given that $t_1,t_2\in \vst$, $\circ \in \{<,=\}$, 
%        and $(\tll(t_1),\hdd(t_2),\circ) \in R$.       
%%    \item\label{ii:forall} $(\forall x. \phi) \in \tau$, and
%%        $\hdd(\forall x. \phi)=\tll(\forall x. \phi)=x$, 
%%        given that $\phi \in \tau$, $x\in X$, and 
%%        $\exists a \in A. (x,A,[~]) \in R$.
%\end{enumerate}
%\item\label{i:tau} $\tau^K = \tau^K_b \cup \tau^K_s$. 
%\item\label{i:exttau} 
%\item Quantified extension to $\tau^K$
%\begin{enumerate}
%\item $\forall \bar{x}. \phi(\bar{x}) \rightarrow \psi(\bar{x})
%\in \exists\forall_i\tau^K$, where $\phi(\bar{x})$ is a Boolean formula over
%terms from $\tau^K_b$, $\psi(\bar{x})$ is a Boolean formula over terms from 
%$\tau^K_b$, and $\bar{x}$ is a vector of variables from $X$ such that
%$\forall x \in \bar{x} \exists a\in A. (x,a,[~])\in R$.
%In addition, $\forall x \in \bar{x}$ the application of $(x,.,\circ), \circ \in
%\{+,-,[~]\}$ is not allowed in $\phi(\bar{x})$.
%%    \item\label{ii:forall} $(\forall x. \phi) \in \tau$, and
%%        $\hdd(\forall x. \phi)=\tll(\forall x. \phi)=x$, 
%%        given that $\phi \in \tau$, $x\in X$, and 
%%        $\exists a \in A. (x,A,[~]) \in R$.
%\end{enumerate}
%\end{enumerate}
%
%
%The theory $\tau^K$ is decidable since it is a quanitifier free, equality
%theory with uninterpreted functions encoding the arrays. 
%In particular, the decidability of a Boolan formula $\phi$ under $\tau^K$ in $D$
%is equisatisfiable to the decidability of $\phi$ in a finite domain $D^f$ where
%the maximum array size is bounded by $|\vit|+1 \le K(2|X| + 2|C| + 1) + 1$; 
%enough values to discriminate all possible index terms. 
%
%Each array read $a[t]$ can have up to $|\vit|+1$ scalar values. 
%Thus we need $K(|X|+|C|+ |\vit|.|A|)$ scalar values in $D^f$ to distinguish
%all possible scalar terms. 
%
%From theorem 2 in ~\cite{Brdly06}, we have that an array property formula
%$\phi \in \exists\forall_i\tau^K$ is reducible to a quantifier free
%formula $\psi$ under $\tau^k$ with a polynomial expansion in the size of $\phi$
%and without a change in $\vit$, $\vst$, $\tau^K_b$, and $\tau^K_s$. 
%Thus the same bound on the domain $D^f$ applies. 
%
%
%
%\begin{figure}[t!]
%\center{
%\fbox{\parbox{\textwidth}{
%\begin{tabbing}
%mm\=mm\=mm\=mm\=mm\=mm\= \kill
%\textbf{ComputeEquivalence($\vocrm$)} \cmnt abstract version \\[1ex]
%
%let $G=\{g_1,g_2,\ldots,g_m\} = \vocrm$;\\
%define $E_G\df (g_1 \ev b_1) \land (g_2 \ev b_2) \cdots \land (g_m \ev b_m)$
%where $b_1,\ldots,b_n$ are fresh boolean variables.\\
%define $V$ to be the set of mappings from $\set{b_1,\ldots,b_n}$ to $\{\tt,
%\ff\}$.\\
%let $W=V$;\\
%let $K=\{(v_1,v_2): (v_1,v_2) \in W\times W \land v_1\not= v_2)\}$;\\
%
%\FOREACH $(v_1,v_2) \in K$\\
%  let $[v_1] \df \{\sg : \sg \sat \E_{v_1}\}$;\\
%  if $[v_1] = \{\}$ then \cmnt SMT returned unsat \\
%  \>let $U = \mathit{unsatcore}(\E_{v_1})$;\\
%  \>let $W = W - \{v: [v] \subseteq [U]\}$;\\
%  \>let $K=\{(u_1,u_2): (u_1,u_2) \in W\times W \land u_1\not= u_2)\}$;\\
%  \>\CONTINUE;\\
%
%  let $[v_2] \df \{\sg : \sg \sat \E_{v_1}\}$;\\
%  if $[v_2] = \{\}$ then \cmnt SMT returned unsat \\
%  \>let $U = \mathit{unsatcore}(\E_{v_2})$;\\
%  \>let $W = W - \{v: [v] \subseteq [U]\}$;\\
%  \>let $K=\{(u_1,u_2): (u_1,u_2) \in W\times W \land u_1\not= u_2)\}$;\\
%  \>\CONTINUE;\\
%
%  let $\sg_1 \in [v_1]$;\\
%  let $\sg_2 \in [v_2]$;\\
%  if $\sg_1 \ev \sg_2$ then \cmnt query the user whether $\sg_1$ and $\sg_2$ are
%equivalent\\
%  \> let $W = W - \{v_1\} - \{v_2\} + \{v_1\lor v_2\}$;\\
%  \>let $K=\{(u_1,u_2): (u_1,u_2) \in W\times W \land u_1\not= u_2)\}$;\\
%
%\ENDFOR\\
%\RETURN(``$W$ as an equivalence class that satisfies the axiom.'');\\
%\end{tabbing}
%\vspace{-1em}
%}}}
%\caption{\textbf{ComputeEquivalence($\vocrm$)}}
%%\vspace{-.5em}
%\label{a:buildequivalence}
%\end{figure}
%
%
%\subsection{earlier tries before using bradley 2006}
%
%Let $X=\{x_1,x_2,\ldots, x_n\}$ be a set of variables, and let 
%$T=\{\mathit{sc},\mathit{in},\mathit{asc},\mathit{ain}\}$ be a set of variable types where 
%$\mathit{sc}$ denotes a scalar, $\mathit{in}$ denotes an index, 
%$\mathit{asc}$ denotes an array of scalars type,
%and $\mathit{ain}$ denotes an array of indices type. 
%The function $\mathit{type}: X\mapsto T$ maps variables to types.
%
%We define the set of index terms ${\cal T}_I$ to be the following.
%\begin{itemize}
%\item $c$ where $c\in\{1,2,\ldots,N\}$ is a constant scalar.
%\item $x$ such that $T(x)= \mathit{in}$.
%\item $|x|$ denoting the size of the array $x$ where $T(x)\in \{\mathit{asc},\mathit{ain}\}$.
%\item $t_1 \circ t_2$ where $\circ \in \{+,-,*,/,\%\}$ denotes an arithmetic operation and $t_1,t_2\in {\cal T}_I$.
%\item $x[t]$ such that $t{\cal T}_I$ and $T(x) = \mathit{ain}$.
%\end{itemize}
%
%We define the set of scalar terms ${\cal T}_S$ to be the following.
%\begin{itemize}
%\item $c$ where $c=\{1,2,\ldots,N\}$ is a constant scalar.
%\item $x$ such that $T(x)= \mathit{sc}$.
%\item $t_1 \circ t_2$ where $\circ \in \{+,-,*,/,\%\}$ denotes an arithmetic operation and $t_1,t_2\in {\cal T}_S$.
%\item $x[t]$ such that $t{\cal T}_I$ and $T(x) = \mathit{asc}$.
%\end{itemize}
%
%We define the set of atomic vocabulary clauses $\mathit{voc}_a$ to be all clauses of the following form. 
%\begin{itemize}
%\item $t_1 \circ t_2$  where $\circ\in\{<,=\} $ and $t_1,t_2\in {\cal T}_I$. 
%\item $t_1 \circ t_2$  where $\circ\in\{<,=\} $ and $t_1,t_2\in {\cal T}_S$. 
%\item $x_i=x_j$  where $T(x_i) = \mathit{sc}$ and $T(x_j) = \mathit{in}$.
%\item $x_i=x_j$  where $T(x_i) = \mathit{asc}$ and $T(x_j) = \mathit{ain}$.
%\end{itemize}
%
%The last two rules allow identity relations between the index and the scalar spaces which are useful 
%to specify index dependent data properties in algorithms such as selection algorithms. 
%
%We define $\mathit{voc}_a^M$ to be a finite set of 
%atomic vocabulary clauses of size smaller than $M$;
%$\mathit{voc}_a^M$ is finite 
%since $\{1,2,\ldots,N\}$ is a finite set of constants.
%
%\subsection{Reduce $\mathit{voc}_a^M$ using SMT}
%Some clauses in $\mathit{voc}_a^M$ are redundant.
%That is they are not necessary to discriminate between input valuations. 
%Let $D_1,D_2,\ldots, D_n$ be the domains of $x_1,x_2,\ldots,x_n$,
%then $D=D_1\times D_2 \times \ldots \times D_n$ is the set of 
%all variable valuations. 
%We say two sets of vocabulary clauses $G=\{g_1,g_2,\ldots,g_m\}$ and $G^-=G - \{g_m\}$
%are equivalent ($g_m$ is redundant) iff
%
%\begin{equation}
%\neg \exists \Phi \in L_{G^-} \exists d \in D. (\Phi \wedge g_m)(d) \not= (\Phi\wedge \neg g_m)(d).
%\label{eq:reducevoc}
%\end{equation}
%
%We encode Equation~\ref{eq:reducevoc} into an SMT check by introducing $m-1$ Boolean variables
%$b_1,b_2,\ldots,b_{m-1}$ and checking the following formula.
%\begin{equation}
%b_1=g_1\wedge b_2=g_2 \wedge b_{m-1}=g_{m-1} \rightarrow g_m \not= \neg g_m.
%\end{equation}
%
%We can apply the SMT check for Equation~\ref{eq:reducevoc} for at most $m^2$ 
%times to compute a reduced vocabulary from $\mathit{voc}_a^M$. 
%
%\subsection{Search for Adequate vocabulary  in $\mathit{voc}_a^M(x_1,x_2,\ldots,x_n)$ }
%
%The problem of finding an adequate vocabulary $\mathit{voc}_q \subset \mathit{voc}_a^M$ is a search problem 
%for an adequate subset of $\mathit{voc}_a^M$. 
%Given an equivalence relation defined 
%with $\{p_1,p_2,\ldots,p_k\} \subset \mathit{voc}_a^M(x_1,x_1',x_2,x_2',\ldots, x_n,x_n')$ 
%
%\subsection{Search for Equivalence Basis}
%
%
%
%
%

